Rank and run-time aware compression of NLP Applications

Sequence model based NLP applications can be large. Yet, many applications that benefit from them run on small devices with very limited compute and storage capabilities, while still having run-time constraints. As a result, there is a need for a compression technique that can achieve significant compression without negatively impacting inference run-time and task accuracy. This paper proposes a new compression technique called Hybrid Matrix Factorization that achieves this dual objective. HMF improves low-rank matrix factorization (LMF) techniques by doubling the rank of the matrix using an intelligent hybrid-structure leading to better accuracy than LMF. Further, by preserving dense matrices, it leads to faster inference run-time than pruning or structure matrix based compression technique. We evaluate the impact of this technique on 5 NLP benchmarks across multiple tasks (Translation, Intent Detection, Language Modeling) and show that for similar accuracy values and compression factors, HMF can achieve more than 2.32x faster inference run-time than pruning and 16.77% better accuracy than LMF.

==> Main/ResultsSubFigure.tex <==
\iffalse
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{Figures/NMT.pdf}
\caption{Accuracy vs speedup for the NMT\_VIEN network comparing the baseline with a smaller baseline and the baseline compressed using different compression schemes at varying compression factors. Speed-up values $>1$ indicate a decrease in inference run-time and values $<1$ indicate an increase in inference run-time. For each compression factor, the compression scheme that is most to the top-right is the ideal choice and is highlighted in bold italics. P = Pruning, LMF = Low rank matrix factorization, HLF = Hybrid matrix decomposition, SB = Smaller baseline. The best way to view this figure is to focus on a compression point and see how the Pareto curve of accuracy vs speed-up changes as we add HLF. For all 3 compression points, HLF provides a viable alternative to both pruning and LMF. \textbf{HLF improves the BLEU score achieved by LMF by 2.3\% to 4.5\% and by Small Baseline by 2.8\% to 4.1\%. At the same time, HLF improves the inference run-time over pruning by $1.5-1.74\times$}}
\label{fig:nmt}
\end{figure}

\begin{figure}
\includegraphics[width=\columnwidth]{Figures/PTB-LM-Medium-3Comp.pdf}
\caption{Perplexity vs speedup for PTB-LM (Medium) network comparing the baseline with a smaller baseline and the baseline compressed using different compression schemes at varying compression factors. Speed-up values $>1$ indicate a decrease in inference run-time and values $<1$ indicate an increase in inference run-time. \textit{In case of perplexity, lower values are better}. Thus, for each compression factor, the compression scheme that is most to the bottom-right is the ideal choice and is highlighted in bold italics. P = Pruning, LMF = Low rank matrix factorization, HLF = Hybrid matrix decomposition, SB = Smaller baseline. The best way to view this figure is to focus on a compression point and see how the Pareto curve of perplexity vs speed-up changes as we add HLF. HLF provides a viable alternative to both pruning and LMF at compression factors of 2.5x, 3.0x and 5x. \textbf{HLF can achieve 17\% better perplexity than LMF, 9\% better perplexity than small baseline and $2.32\times$ better inference run-time than pruning.}}
\label{fig:ptblm_med}

\end{figure}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{Figures/TextClassification.pdf}
\caption{Accuracy vs speedup for the text classification task on dbpedia database comparing the baseline with a smaller baseline and the baseline compressed using different compression schemes at varying compression factors. Speed-up values $>1$ indicate a decrease in inference run-time and values $<1$ indicate an increase in inference run-time. For each compression factor, the compression scheme that is most to the top-right is the ideal choice and is highlighted in bold italics. P = Pruning, LMF = Low rank matrix factorization, HLF = Hybrid matrix decomposition, SB = Smaller baseline. The best way to view this figure is to focus on a compression point and see how the Pareto curve of accuracy vs speed-up changes as we add HLF. For all 3 compression points, HLF provides netter accuracy than LMF and SB and better run-time than pruning. \textbf{HLF can improve the accuracy achieved by LMF by up-to 1.2\% and SB by up-to 1.3\% and improve the run-time achieved by pruning by up-to $1.2\times$}}
\label{fig:textclass}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{Figures/SlotFilling.pdf}
\caption{Accuracy vs speedup for the ATIS Slot Detection task comparing the baseline with a smaller baseline and the baseline compressed using different compression schemes at varying compression factors. Speed-up values $>1$ indicate a decrease in inference run-time and values $<1$ indicate an increase in inference run-time. For each compression factor, the compression scheme that is most to the top-right is the ideal choice and is highlighted in bold italics. P = Pruning, LMF = Low rank matrix factorization, HLF = Hybrid matrix decomposition, SB = Smaller baseline. The best way to view this figure is to focus on a compression point and see how the Pareto curve of accuracy vs speed-up changes as we add HLF. For all 3 compression points, HLF provides netter accuracy than LMF and SB and better run-time than pruning. \textbf{HLF can improve the accuracy achieved by LMF and SB by up-to 1.2\% and improve the run-time achieved by pruning by up-to $1.26\times$}}
\label{fig:slot}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{Figures/IntentDetection.pdf}
\caption{Accuracy vs speedup for the ATIS Intent Detection task comparing the baseline with a smaller baseline and the baseline compressed using different compression schemes at varying compression factors. Speed-up values $>1$ indicate a decrease in inference run-time and values $<1$ indicate an increase in inference run-time. For each compression factor, the compression scheme that is most to the top-right is the ideal choice and is highlighted in bold italics. P = Pruning, LMF = Low rank matrix factorization, HLF = Hybrid matrix decomposition, SB = Smaller baseline. The best way to view this figure is to focus on a compression point and see how the Pareto curve of accuracy vs speed-up changes as we add HLF. For all 3 compression points, HLF provides better accuracy than LMF and SB and better run-time than pruning. \textbf{HLF can improve the accuracy achieved by LMF and SB by up-to 1\% and improve the run-time achieved by pruning by up-to $1.26\times$} }
\label{fig:intent}
\end{figure}
\fi

\begin{figure*}
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.475\linewidth]{Figures/NMT.pdf}%
        \hfill
        \includegraphics[width=0.475\linewidth]{Figures/TextClassification.pdf}
        \caption{\textit{(Left)Language Translation:} For all 3 compression points, HLF provides a viable alternative to both pruning and LMF. \textbf{HLF improves the BLEU score achieved by LMF by 2.3\% to 4.5\% and by Small Baseline by 2.8\% to 4.1\%. At the same time, HLF improves the inference run-time over pruning by $1.5-1.74\times$}.\\ \textit{(Right)Text Classification:} For all 3 compression points, HLF provides netter accuracy than LMF and SB and better run-time than pruning. \textbf{HLF can improve the accuracy achieved by LMF by up-to 1.2\% and SB by up-to 1.3\% and improve the run-time achieved by pruning by up-to $1.2\times$}}
        \label{fig:nmt}
        \label{fig:textclass}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.475\linewidth]{Figures/SlotFilling.pdf}%
        \hfill
        \includegraphics[width=0.475\linewidth]{Figures/IntentDetection.pdf}
        \caption{\textit{(Left) Slot Filling}: For all 3 compression points, HLF provides better accuracy than LMF and SB and better run-time than pruning. \textbf{HLF can improve the accuracy achieved by LMF and SB by up-to 1.2\% and improve the run-time achieved by pruning by up-to $1.26\times$}.\\ \textit{(Right) Intent Detection}: For all 3 compression points, HLF provides better accuracy than LMF and SB and better run-time than pruning. \textbf{HLF can improve the accuracy achieved by LMF and SB by up-to 1\% and improve the run-time achieved by pruning by up-to $1.26\times$}}
        \label{fig:intent}
        \label{fig:slot}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.475\textwidth]{Figures/PTB-LM-Medium-3Comp.pdf}
    \caption{Language Modeling: HLF provides a viable alternative to both pruning and LMF at compression factors of 2.5x, 3.0x and 5x. \textbf{HLF can achieve 17\% better perplexity than LMF, 9\% better perplexity than small baseline and $2.32\times$ better inference run-time than pruning.}}
    \label{fig:ptblm_med}
\end{subfigure}
    \caption{Accuracy vs Speed-up over baseline  comparing the baseline with a smaller baseline and the baseline compressed using different compression schemes at varying compression factors. Speed-up values $>1$ indicate a decrease in inference run-time and values $<1$ indicate an increase in inference run-time. \textbf{For each compression factor, the compression scheme that is most to the top-right is the ideal choice}. \textit{In case of perplexity, lower values are better}. Thus, the graphs are plotted in a slightly different way to still adhere to the fact that the most ideal choice of compression is in the top-right corner. P = Pruning, LMF = Low rank matrix factorization, HLF = Hybrid matrix decomposition, SB = Smaller baseline. The best way to view this figure is to focus on a compression point and see how the Pareto curve of Speed-up vs Accuracy over baseline  changes as we add HLF.}
\end{figure*}
